dRTI: Directional Radio Tomographic Imaging

Radio tomographic imaging (RTI) enables device free localisation of people and objects in many challenging environments and situations. Its basic principle is to detect the changes in the statistics of some radio quality measurements in order to infer the presence of people and objects in the radio path. However, the localisation accuracy of RTI suffers from complicated radio propagation behaviours such as multipath fading and shadowing. In order to improve RTI localisation accuracy, we propose to use inexpensive and energy efficient electronically switched directional (ESD) antennas to improve the quality of radio link behaviour observations, and therefore, the localisation accuracy of RTI. We implement a directional RTI (dRTI) system to understand how directional antennas can be used to improve RTI localisation accuracy. We also study the impact of the choice of antenna directions on the localisation accuracy of dRTI and propose methods to effectively choose informative antenna directions to improve localisation accuracy while reducing overhead. We evaluate the performance of dRTI in diverse indoor environments and show that dRTI significantly outperforms the existing RTI localisation methods based on omni-directional antennas.

==> Tex/related_spida.tex <==
\subsection{Direction Antenna}
Electronically Switched Directional antennas allow software based control of the direction of the maximum antenna gain. These have been shown feasible for the resource constrained environment of the low power sensor network. The feasibility has been demonstrated by Nilsson~\cite{nilsson09directional}, Prieditis et al. and Giorgetti et al.~\cite{giorgetti07directional} with their prototype antennas. Giorgetti et al.  discuss a four beam patch antenna. The antenna consists of four planar patch antennas arranged in a box like structure that can be controlled electronically. They integrate the antenna with TelosB nodes~\cite{polastre05telos}, and demonstrated increased transmission range, decreased signal variability and interference suppression from IEEE 802.11 networks. The ESD antennas discussed by Nilsson  and Prieditis et al. are based on the concept of Electrically Switched Parasitic Element (ESPE). These antennas consists a of central monopole antenna surrounded by a number of parasitic elements. The reactance between the elements can be electronically controlled. Prieditis et al.  designed an ESPE based antenna and integrated it with TelosB nodes. They observed improved communication range at the same energy cost. Nilsson designed the Sics Parasitic Interference Directional Antenna (SPIDA). SPIDA is an implementation of the ESPE design. SPIDA's six parasitic elements can be individually grounded or isolated. When all parasitic elements are isolated the antenna is configured in omni-directional mode. When all elements are grounded except one, the direction of the maximum antenna gain is towards the direction of the isolated element. \"Ostr\"om added software-based control to SPIDA and demonstrated that the SPIDA prototype concentrates the radiated power in the given directions~\cite{Ostrom:2010:EES:1947841.1947856}. 

